Convolutional Tensor-Train LSTM for Spatio-temporal Learning

Learning from spatio-temporal data has numerous applications such as human-behavior analysis, object tracking, video compression, and physics simulation.However, existing methods still perform poorly on challenging video tasks such as long-term forecasting. This is because these kinds of challenging tasks require learning long-term spatio-temporal correlations in the video sequence. In this paper, we propose a higher-order convolutional LSTM model that can efficiently learn these correlations, along with a succinct representations of the history. This is accomplished through a novel tensor train module that performs prediction by combining convolutional features across time. To make this feasible in terms of computation and memory requirements, we propose a novel convolutional tensor-train decomposition of the higher-order model. This decomposition reduces the model complexity by jointly approximating a sequence of convolutional kernels asa low-rank tensor-train factorization. As a result, our model outperforms existing approaches, but uses only a fraction of parameters, including the baseline models.Our results achieve state-of-the-art performance in a wide range of applications and datasets, including the multi-steps video prediction on the Moving-MNIST-2and KTH action datasets as well as early activity recognition on the Something-Something V2 dataset.

==> tex/sub_figure_vis_kth.tex <==
\def\i{483}
\def\j{1323}
\def\ia{483}
\def\ja{1323}
\begin{figure*}[!htbp]
  \centering
  \footnotesize
  \addtolength{\tabcolsep}{-5pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cc}
      input & ground truth (top) / predictions \\ 
      \scriptsize $t = 1 \;\;\;\;\;\;\;\;4\;\;\;\;\;\;\;\;\;\;\;6\;\;\;\;\;\;\;\;\;\;8\;\;\;\;\;\;$ &\scriptsize $11\;\;\;\;\;\;\;\;13\;\;\;\;\;\;\;\;\;\;15\;\;\;\;\;\;\;\;\;17\;\;\;\;\;\;\;\;19\;\;\;\;\;\;\;\;21\;\;\;\;\;\;\;\;\;\;23\;\;\;\;\;\;\;\;\;25\;\;\;\;\;\;\;\;\;\;27\;\;\;\;\;\;\;\;29$ \\
      
      \includegraphics[trim={23cm 9.2cm 4.5cm 0.1cm},clip, height=1cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} &
      \includegraphics[trim={0cm 4.7cm 0.0cm 4.8cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} \\ [-0.2em]

      \raisebox{0.4cm}{E3D} &
      \includegraphics[trim={0cm 0 0.cm 9.0cm},clip, height=1cm,width=10cm]{figs/result_kth/e3d/cmp_\j.png} \\ [-0.2em]

      \raisebox{0.4cm}{\scriptsize \ConvTTLSTM (\(\ell_1 + \ell_2\))} &
      \includegraphics[trim={0cm 0.1cm 0.0cm 9.3cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8/cmp_395_\i.jpg} \\ [-0.2em]

      \raisebox{0.4cm}{{\scriptsize \ConvTTLSTM  (\(\ell_1 + \ell_2 + \ell_{p}\))}} &
      \includegraphics[trim={0cm 0.1cm 0.0cm 9.3cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} \\ [-0.2em]

  \end{tabular}}
  \caption{20 frames prediction on KTH given 10 input frames. Every 2 frames are shown.}
  \label{fig:visual-kth1}
  \vspace{-0.2cm}
\end{figure*}


%<5>-------------------------------------------------
\def\i{844}
\def\j{741}
\def\ia{844}
\def\ja{741}
\begin{figure*}[!htbp]
  \centering
  \footnotesize
  \addtolength{\tabcolsep}{-5pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cc}
      input & ground truth (top) / predictions \\ 
      \scriptsize $t = 1 \;\;\;\;\;\;\;\;4\;\;\;\;\;\;\;\;\;\;\;6\;\;\;\;\;\;\;\;\;\;8\;\;\;\;\;\;$ &\scriptsize $11\;\;\;\;\;\;\;\;13\;\;\;\;\;\;\;\;\;\;15\;\;\;\;\;\;\;\;\;17\;\;\;\;\;\;\;\;19\;\;\;\;\;\;\;\;21\;\;\;\;\;\;\;\;\;\;23\;\;\;\;\;\;\;\;\;25\;\;\;\;\;\;\;\;\;\;27\;\;\;\;\;\;\;\;29$ \\
      
      \includegraphics[trim={23cm 9.2cm 4.5cm 0.1cm},clip, height=1cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} &
      \includegraphics[trim={0cm 4.7cm 0.0cm 4.8cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} \\ [-0.2em]

      \raisebox{0.4cm}{E3D} &
      \includegraphics[trim={0cm 0 0.cm 9.0cm},clip, height=1cm,width=10cm]{figs/result_kth/e3d/cmp_\j.png} \\ [-0.2em]

      \raisebox{0.4cm}{\scriptsize \ConvTTLSTM (\(\ell_1 + \ell_2\))} &
      \includegraphics[trim={0cm 0.1cm 0.0cm 9.3cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8/cmp_395_\i.jpg} \\ [-0.2em]

      \raisebox{0.4cm}{{\scriptsize \ConvTTLSTM  (\(\ell_1 + \ell_2 + \ell_{p}\))}} &
      \includegraphics[trim={0cm 0.1cm 0.0cm 9.3cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} \\ [-0.2em]

  \end{tabular}}
  \caption{20 frames prediction on KTH given 10 input frames. Every 2 frames are shown.}
  \label{fig:visual-kth2}
  \vspace{-0.2cm}
\end{figure*}


%<3>-------------------------------------------------
\def\i{466}
\def\j{3108}
\def\ia{466}
\def\ja{3108}
\begin{figure*}[!htbp]
  \centering
  \footnotesize
  \addtolength{\tabcolsep}{-5pt}
  \resizebox{\textwidth}{!}{
  \begin{tabular}{cc}
      input & ground truth (top) / predictions \\ 
      \scriptsize $t = 1 \;\;\;\;\;\;\;\;4\;\;\;\;\;\;\;\;\;\;\;6\;\;\;\;\;\;\;\;\;\;8\;\;\;\;\;\;$ &\scriptsize $11\;\;\;\;\;\;\;\;13\;\;\;\;\;\;\;\;\;\;15\;\;\;\;\;\;\;\;\;17\;\;\;\;\;\;\;\;19\;\;\;\;\;\;\;\;21\;\;\;\;\;\;\;\;\;\;23\;\;\;\;\;\;\;\;\;25\;\;\;\;\;\;\;\;\;\;27\;\;\;\;\;\;\;\;29$ \\
      
      \includegraphics[trim={23cm 9.2cm 4.5cm 0.1cm},clip, height=1cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} &
      \includegraphics[trim={0cm 4.7cm 0.0cm 4.8cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} \\ [-0.2em]

      \raisebox{0.4cm}{E3D} &
      \includegraphics[trim={0cm 0 0.cm 9.0cm},clip, height=1cm,width=10cm]{figs/result_kth/e3d/cmp_\j.png} \\ [-0.2em]

      \raisebox{0.4cm}{\scriptsize \ConvTTLSTM (\(\ell_1 + \ell_2\))} &
      \includegraphics[trim={0cm 0.1cm 0.0cm 9.3cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8/cmp_395_\i.jpg} \\ [-0.2em]

      \raisebox{0.4cm}{{\scriptsize \ConvTTLSTM  (\(\ell_1 + \ell_2 + \ell_{p}\))}} &
      \includegraphics[trim={0cm 0.1cm 0.0cm 9.3cm},clip, height=1cm,width=10cm]{figs/result_kth/ttv4_o3t3r8_ploss/cmp_395_\i.jpg} \\ [-0.2em]

  \end{tabular}}
  \caption{20 frames prediction on KTH given 10 input frames. Every 2 frames are shown.}
  \label{fig:visual-kth3}
  \vspace{-0.2cm}
\end{figure*}

